Integrating Information About Entities Progressively

Users often have to integrate information about entities from multiple data sources. This task is challenging as each data source may represent information about the same entity in a distinct form, e.g., each data source may use a different name for the same person. Currently, data from different representations are translated into a unified one via lengthy and costly expert attention and tuning. Such methods cannot scale to the rapidly increasing number and variety of available data sources. We demonstrate ProgMap, a entity-matching framework in which data sources learn to collaborate and integrate information about entities on-demand and with minimal expert intervention. The data sources leverage user feedback to improve the accuracy of their collaboration and results. ProgMap also has techniques to reduce the amount of required user feedback to achieve effective matchings.

==> 8.RelatedWork.tex <==
\section{Related Work}
%TODO: SIGMOD paper 
% Researchers have developed effective and efficient reinforcement learning methods for data exploration and answering ill-specified queries over large databases \cite{mccamish2018data}. They have extended reinforcement learning algorithms for effective query answering in usable query interfaces and shown both theoretically and empirically it to improve the effectiveness of query answering in both dynamic and static environment \cite{mccamish2018data}. 
%TODO: current pay-as-you-go techniques using keyword queries

%TODO: language games

%TODO: NIPS workshop and ICLR papers on evoving communications


==> 9.Conclusion.tex <==
\section{Conclusion}
